Versatile Multi-Contact Planning and Control for Legged Loco-Manipulation

Loco-manipulation planning skills are pivotal for expanding the utility of robots in everyday environments. These skills can be assessed based on a system's ability to coordinate complex holistic movements and multiple contact interactions when solving different tasks. However, existing approaches have been merely able to shape such behaviors with hand-crafted state machines, densely engineered rewards, or pre-recorded expert demonstrations. Here, we propose a minimally-guided framework that automatically discovers whole-body trajectories jointly with contact schedules for solving general loco-manipulation tasks in pre-modeled environments. The key insight is that multi-modal problems of this nature can be formulated and treated within the context of integrated Task and Motion Planning (TAMP). An effective bilevel search strategy is achieved by incorporating domain-specific rules and adequately combining the strengths of different planning techniques: trajectory optimization and informed graph search coupled with sampling-based planning. We showcase emergent behaviors for a quadrupedal mobile manipulator exploiting both prehensile and non-prehensile interactions to perform real-world tasks such as opening/closing heavy dishwashers and traversing spring-loaded doors. These behaviors are also deployed on the real system using a two-layer whole-body tracking controller.

==> Sections/Abstract.tex <==
% Place your abstract within the special {sciabstract} environment.
%\begin{sciabstract}
% \parbox{0.85\textwidth}{  
% \bf\vspace{10pt}
% This document presents a number of hints about how to set up your
%   {\it Science\/} paper in \LaTeX\ .  We provide a template file,
%   \texttt{scifile.tex}, that you can use to set up the \LaTeX\ source
%   for your article.  An example of the style is the special
%   \texttt{\{sciabstract\}} environment used to set up the abstract you
%   see here.}
%\end{sciabstract}

%\begin{sciabstract}
\parbox{0.85\textwidth}{\textbf{Loco-manipulation planning skills are pivotal for expanding the utility of robots in everyday environments. These skills can be assessed based on a system's ability to coordinate complex holistic movements and multiple contact interactions when solving different tasks. However, existing approaches have been merely able to shape such behaviors with hand-crafted state machines, densely engineered rewards, or pre-recorded expert demonstrations. Here, we propose a minimally-guided framework that automatically discovers whole-body trajectories jointly with contact schedules for solving general loco-manipulation tasks in pre-modeled environments. The key insight is that multi-modal problems of this nature can be modeled within the context of integrated Task and Motion Planning (TAMP), resulting in a tractable bilevel optimization formulation. An effective bilevel search strategy is achieved owing to the fusion of domain-specific rules with the well-established strengths of different planning techniques: trajectory optimization and informed graph search, coupled with sampling-based planning. We showcase emergent behaviors for a quadrupedal mobile manipulator exploiting both prehensile and non-prehensile interactions to perform real-world tasks such as opening/closing heavy dishwashers and traversing spring-loaded doors. These behaviors are also deployed on the real system using a two-layer whole-body tracking controller.}}


% This paper addresses the problem of trajectory optimization for multi-limbed floating-base systems performing loco-manipulation tasks with multiple contact switches involved. The proposed framework is provided a user-defined set of robot end-effectors and object affordances, in addition to a high-level task specification that is defined in the form of a robot-centric or object-centric sparse goal region. Subsequently, the underlying planner automatically discovers feasible contact schedules jointly with high-fidelity trajectories that connect the start state to the goal. The key insight is that multi-modal problems of this nature can be formulated and treated within the well-established context of Task and Motion Planning (TAMP). An effective search strategy is achieved by making use of domain-specific knowledge and adequately exploiting the strengths of different planning techniques, namely trajectory optimization and informed graph search coupled with sampling-based planning. A wide range of multi-contact manipulation tasks involving both prehensile and non-prehensile interaction phases can be covered with this approach. For example, we showcase the following emergent behaviors: turning a large valve using multiple regrasps, opening/closing a dishwasher by exploiting various contact interactions, opening a spring-loaded door with a sequence similar to \cite{SpotWithArm}, and navigating while manipulating a movable obstacle. The generated solutions are demonstrated to be physically consistent by executing some of them on a real quadrupedal mobile manipulator using a two-layer whole-body tracking controller.


%\end{sciabstract}

% NOTE: The abstract should be a single paragraph, not to exceed 250 words and ideally closer to 200, written in plain language that a general reader can understand. It should include
%     An opening sentence that states the question/problem addressed by the research AND
%     Enough background content to give context to the study AND
%     A brief statement of primary results AND
%     A short concluding sentence.
% Do not include citations or undefined abbreviations in the abstract. Any abbreviations that appear in the title should be defined in the abstract.

==> Sections/Captions.tex <==
\noindent Fig.1. \textbf{Planning and control architecture for multi-contact loco-manipulation.} (\textbf{A}) The user provides the offline planner with a basic high-level description of the scene: A sparse task specification given by a start state and a target goal region, dynamic models of the robot and the object, specification and classification of robot end-effectors and object affordances. (\textbf{B}) The central element in the offline planner is (\textbf{i}) a sampling-based bilevel optimization that gradually grows a tree of mode-invariant short-horizon trajectories seeking an optimal multi-modal sequence that reaches the goal region. Modes are determined by contact state and action pairs $\langle\bm s_k, \bm a_k\rangle$ that encode for each end-effector whether it is a closed, open, or switching manipulation contact, and the object contact it is interacting with. Each color corresponds to a specific contact state, and consecutive color variations indicate a contact switch. (\textbf{ii}) The second component in the planner is a long-horizon trajectory optimization that is warm-started with the bilevel optimization solution. It uses the same contact schedule and only polishes the continuous part. (\textbf{C}) To deploy multi-contact behaviors, the online module relies on an MPC-based whole-body controller that tracks the offline references. (\textbf{D}) With such a framework, complex behaviors that require exploiting multiple contact interactions, such as traversing a spring-loaded pull door, can be rapidly generated (i.e., often requires less than 1 minute on an ordinary laptop), and reliably executed with a real quadrupedal mobile manipulator.

\noindent Movie 1 Summary of the results and methods.

\noindent Fig.2. \textbf{Validation of loco-manipulation planner.} (\textbf{A}) Illustration of two object-centric and two robot-centric tasks: i) dishwasher manipulation (\href{https://youtu.be/hgIanclikFI}{Movie S1}), ii) valve manipulation (\href{https://youtu.be/2YhAm4o7w3c}{Movie S2}), iii) traversal of an obstructing movable obstacle (\href{https://youtu.be/haS3y2uZDH0}{Movie S3}), iv) traversal of a large articulated object  (\href{https://youtu.be/-vLXUrBMbMI}{Movie S4}). Diverse behaviors emerge highlighting the planner's adaptability to variations in each task. \textbf{Task 1:} (\textbf{B}) Different start states and goal regions (opening vs. closing) (\textbf{C}) Opening with different joint limits and self-collision constraints for the robot. \textbf{Task 2:} (\textbf{D}) and (\textbf{E}) Different numbers, types and locations of object contacts, for two varying valve heights (low vs. high). \textbf{Task 3:} (\textbf{F}) and (\textbf{G}) Different robot end-effector contacts enabled for manipulation (enabled arm contact vs. blocked arm contact). \textbf{Task 4:} (\textbf{H}) and (\textbf{I}) Different joint limits (push vs. pull) and dynamics (recoil vs. no recoil) for the object.

\noindent Fig.3. \textbf{Hardware experiments -- Feasibility verification for push door with recoil behaviors.} (\textbf{A} to \textbf{C}) Different manipulation schedules discovered and executed to solve the same task. Red: prehensile interaction with handle, Green: nonprehensile interaction with surface. ARM: 6-DoF robotic arm, LF: left front leg, RF: right front leg, LH: left hind leg, RH: right hind leg. The numbers on the schedules indicate certain instants captured in the corresponding snapshots.

\noindent Fig.4. \textbf{Hardware experiments -- Feasibility verification for pull door with recoil behaviors.} (\textbf{A}) The different gait schedules adopted in this scenario. Left: normal trot and fast trot; Right: standing trot. LF: left front leg, RF: right front leg, LH: left hind leg, RH: right hind leg. (\textbf{B}) Motion tracking accuracy of the base pose and manipulating limbs.

\noindent Fig.5. \textbf{Hardware experiments -- Feasibility verification for dishwasher manipulation behaviors.} (\textbf{A}) and (\textbf{B}) Image sequence of executed multi-contact behaviors for manipulating a heavy dishwasher with high stiction highlighting different interaction phases: opening and closing maneuvers, respectively. (\textbf{C}) Motion tracking accuracy and exerted manipulation forces corresponding to the arm during the opening scenario. (\textbf{D}) and (\textbf{E}) Motion tracking accuracy and exerted manipulation forces corresponding to the arm and left front leg, respectively, during the closing scenario.

==> Sections/SupplementaryMaterials.tex <==
\section*{SUPPLEMENTARY MATERIALS}
%Here you should list the contents of your Supplementary Materials -- below is an example. 
%You should include a list of Supplementary figures, Tables, and any references that appear only in the SM. 
%Note that the reference numbering continues from the main text to the SM.
% In the example below, Refs. 4-10 were cited only in the SM.

% Include dynamics and constraints used inside the OCP? 

\noindent 
Section S1. Nomenclature \\
Section S2. Contact-driven OCP formulation: Dynamics\\
Section S3. Contact-driven OCP formulation: Constraints\\
Section S4. Contact-driven OCP formulation: Cost Function\\
Section S5. Reference generation \\
Section S6. Implementation details\\
Section S7. Ablation study over framework components\\
Section S8. Towards real-world deployment\\
Fig. S1. Robot-Object reference frames.\\
Fig. S2. Robot-Object collision bodies.\\
Fig. S3. Ablation study over framework components.\\
Fig. S4. Block diagram detailing MPC-WBC interconnections.\\
Table S1. Objects model parameters.  \\
Table S2. Inner-Level OCP cost weights. \\
Table S3. Task-dependent hyperparameters for reference generation. \\
Table S4. Task-independent hyperparameters for bilevel search.\\
Table S5. Task-independent hyperparameters for NNS metric and auxiliary strategies.\\
Table S6. MPC cost weights.\\
Table S7. WBC prioritized tasks list. \\
Movie S1. Generated behaviors for dishwasher manipulation task.\\
Movie S2. Generated behaviors for valve manipulation task.\\
Movie S3. Generated behaviors for movable obstacle traversal task.\\
Movie S4. Generated behaviors for door traversal task.\\
Movie S5. Ablation study over framework components.\\
Movie S6. Demonstration of inherent robustness.\\  
Movie S7. Towards autonomous door traversal.
